Determination of the Point-Spread Function for the Fermi Large Area Telescope from On-orbit Data and Limits on Pair Halos of Active Galactic Nuclei

The Large Area Telescope (LAT) on the Fermi Gamma-ray Space Telescope is a pair-conversion telescope designed to detect photons with energies from 20 MeV to > 300 GeV. The pre-launch response functions of the LAT were determined through extensive Monte Carlo simulations and beam tests. The point-spread function (PSF) characterizing the angular distribution of reconstructed photons as a function of energy and geometry in the detector is determined here from two years of on-orbit data by examining the distributions of \gamma rays from pulsars and active galactic nuclei (AGN). Above 3 GeV, the PSF is found to be broader than the pre-launch PSF. We checked for dependence of the PSF on the class of \gamma-ray source and observation epoch and found none. We also investigated several possible spatial models for pair-halo emission around BL Lac AGN. We found no evidence for a component with spatial extension larger than the PSF and set upper limits on the amplitude of halo emission in stacked images of low and high redshift BL Lac AGN and the TeV blazars 1ES0229+200 and 1ES0347-121.

==> Tables/back.tex <==
\begin{table}[8]\footnotesize
\begin{center}
\caption{Back PSF parameters}
\begin{tabular}{|l|rcrrrrrr|}
\hline
\multicolumn{9}{|c|}{1.0--1.7 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 22884 & 14405 & 0.260 & 1.62 & 1.07 & 0.89 & 5.15 & 2.26 \\
Geminga & 11526 & 1201  & 0.280 & 1.71 & 1.04 & 0.92 & 4.29 & 2.24 \\
Crab & 3036 & 9511 & 0.272 & 1.68 & 1.04 & 0.94 & 4.44 & 2.28 \\
All Pulsars & 37103 & 32909 & 0.273 & 1.72 & 1.00 & -- & 4.08 & -- \\
AGN & 3569 & 26488 & 0.249 & 1.62 & 1.03 & -- & 5.01 & -- \\
\hline
\multicolumn{9}{|c|}{1.7--3.2 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 11134 & 1971 & 0.195 & 1.82 & 0.64 & 0.59 & 2.27 & 1.42 \\
Geminga & 6408 & 498 & 0.204 & 1.93 & 0.62 & 0.61 & 1.97 & 1.40\\
Crab & 1421 & 1095 & 0.207 & 1.96 & 0.62 & 0.60 & 1.91 & 1.41 \\
All Pulsars & 18977 & 3550 & 0.198 & 1.86 & 0.64 & -- & 2.15 & --\\
AGN & 2211 & 12518 & 0.198 & 1.94 & 0.60 & -- & 1.89 & -- \\
\hline
\multicolumn{9}{|c|}{3.2--5.6 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 4306 & 854 & 0.145 & 1.94 & 0.44 & 0.41 & 1.37 & 0.97 \\
Geminga & 2352 & 234 & 0.152 & 2.08 & 0.42 & 0.44 & 1.20 & 0.90\\
Crab & 637 & 450 & 0.166 & 2.39 & 0.41 & 0.42 & 1.00 & 1.25 \\
All Pulsars & 7277 & 1556 & 0.149 & 2.02 & 0.43 & -- & 1.26 & -- \\
AGN & 1375 & 5362 & 0.154 & 1.99 & 0.45 & -- & 1.37 & -- \\
\hline
\multicolumn{9}{|c|}{5.6--10.0 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 1279 & 354 & 0.123 & 1.91 & 0.38 & 0.38 & 1.23 & 0.91\\
Geminga & 606 & 105 & 0.127 & 2.16 & 0.34 & 0.35 & 0.92 & 0.81 \\
Crab & 246 & 167 & 0.148 & 2.80 & 0.33 & 0.38 & 0.73 & 0.79 \\
All & 2127 & 630 & 0.126 & 2.04 & 0.36 & -- & 1.04 & -- \\
AGN & 763 & 2233 & 0.117 & 1.78 & 0.40 & -- & 1.49 & -- \\
\hline
\multicolumn{9}{|c|}{10.0--17.7 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 226 & 94 & 0.105 & 1.60 & 0.45 & 0.39 & 2.25 & 1.19 \\
Geminga & 80 & 29 & 0.084 & 1.55 & 0.39 & 0.30 & 2.22 & 0.92 \\
Crab & 104 & 62 & 0.124 & 2.71 & 0.28 & 0.87 & 0.63 & 1.89 \\
All Pulsars& 408 & 187 & 0.103 & 1.74 & 0.37 & -- & 1.45 & -- \\
AGN & 427 & 889 & 0.091 & 1.63 & 0.37 & -- & 1.74 & -- \\
\hline
\multicolumn{9}{|c|}{17.7--31.6 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 36 & 55 & 0.069 & 1.38 & 0.49 & 0.44 & 5.64 & 1.37 \\
Geminga & 6 & 11 & 0.066 & 1.94 & 0.20 & 1.18 & 0.62 & 1.71 \\
Crab & 37 & 33 & 0.066 & 2.82 & 0.15 & 0.88 & 0.32 & 1.31 \\
All Pulsars & 75 & 103 & 0.061 & 1.77 & 0.21 & -- & 0.79 & -- \\
AGN & 204 & 505 & 0.061 & 1.65 & 0.24 & -- & 1.12 & -- \\
\hline
\multicolumn{9}{|c|}{31.6--100.0 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & -- & -- & -- & -- & -- & -- & -- & -- \\
Geminga & -- & -- & -- & -- & -- & -- & -- & -- \\
Crab & 34 & 20 & 0.084 & 1.79 & 0.28 & -- & 1.04 & -- \\
All Pulsars & 46 & 75 & 0.083 & 1.58 & 0.37 & -- & 1.94 & -- \\
AGN & 193 & 436 & 0.060 & 1.88 & 0.19 & -- & 0.62 & -- \\
\hline
\end{tabular}
\tablecomments{$R_{X}^1$ is the X\% containment radius determined by the stacking analysis. $R_{X}^2$ is the containment determined by background subtraction.}
\end{center}
\end{table}

==> Tables/comp.tex <==
\begin{table}[8]\footnotesize
\caption{Comparison between parameters derived from pulsars (PSR) and blazars (AGN)}
\begin{center}
\begin{tabular}{|l|rrr|rrr|}
\hline
\multicolumn{7}{|c|}{Point-Spread Function Containment} \\
\hline
E (GeV) & PSR $R_{68}^1 (deg)$ & PSR $R_{68}^2 (deg)$ & AGN $R_{68} (deg)$ & PSR $R_{95} (deg)$ & PSR $R_{95}^2 (deg)$ & AGN $R_{95} (deg)$ \\
\hline
1.0--1.7 & 0.50 +/-- 0.01 & 0.48 +/-- 0.01 & 0.49 +/-- 0.02 & 1.56 +/-- 0.05 & 1.22 +/-- 0.03 & 1.49 +/-- 0.25 \\
1.7--3.2 & 0.32 +/-- 0.01 & 0.31 +/-- 0.01 & 0.31 +/-- 0.01 & 0.88 +/-- 0.02 & 0.76 +/-- 0.02 & 0.87 +/-- 0.10 \\
3.2--5.6 & 0.22 +/-- 0.01 & 0.21 +/-- 0.01 & 0.22 +/-- 0.01 & 0.53 +/-- 0.01 & 0.51 +/-- 0.03 & 0.60 +/-- 0.07 \\
5.6--10.0 & 0.18 +/-- 0.01 & 0.18 +/-- 0.01 & 0.18 +/-- 0.01 & 0.50 +/-- 0.03 & 0.49 +/-- 0.04 & 0.53 +/-- 0.08 \\
10.0--17.7 & 0.15 +/-- 0.01 & 0.16 +/-- 0.01 & 0.14 +/-- 0.01 & 0.44 +/-- 0.06 & 0.36 +/-- 0.06 & 0.39 +/-- 0.06 \\
17.7--31.6 & 0.11 +/-- 0.01 & 0.11 +/-- 0.01 & 0.11 +/-- 0.01 & 0.31 +/-- 0.09 & 0.40 +/-- 0.26 & 0.40 +/-- 0.11 \\
31.6--100.0 & 0.13 +/-- 0.09 & -- & 0.09 +/-- 0.01 & 0.73 +/-- 0.61 & -- & 0.38 +/-- 0.14 \\
\hline
\end{tabular}
\tablecomments{$R_{X}^1$ is the X\% containment radius determined by the stacking analysis. $R_{X}^2$ is the containment determined by background subtraction.}
\end{center}
\end{table}
\begin{table}[8]\footnotesize
\caption{Comparison between parameters derived from pulsars (PSR) and blazars (AGN)}
\begin{center}
\begin{tabular}{|l|rrr|rrr|}
\hline
\multicolumn{7}{|c|}{Point-Spread Function Containment} \\
\hline
E (GeV) & PSR $R_{68}^1 (deg)$ & PSR $R_{68}^2 (deg)$ & AGN $R_{68} (deg)$ & PSR $R_{95} (deg)$ & PSR $R_{95}^2 (deg)$ & AGN $R_{95} (deg)$ \\
\hline
1.0--1.7 & 1.00 +/-- 0.02 & 0.89 +/-- 0.01 & 1.03 +/-- 0.21 & 4.08 +/-- 0.24 & 2.26 +/-- 0.09 & 5.01 +/-- 3.61 \\
1.7--3.2 & 0.64 +/-- 0.01 & 0.59 +/-- 0.01 & 0.60 +/-- 0.06 & 2.15 +/-- 0.13 & 1.42 +/-- 0.06 & 1.89 +/-- 0.51 \\
3.2--5.6 & 0.43 +/-- 0.01 & 0.41 +/-- 0.01 & 0.45 +/-- 0.03 & 1.26 +/-- 0.06 & 0.97 +/-- 0.06 & 1.37 +/-- 0.32 \\
5.6--10.0 & 0.36 +/-- 0.01 & 0.38 +/-- 0.02 & 0.40 +/-- 0.04 & 1.04 +/-- 0.08 & 0.91 +/-- 0.09& 1.49 +/-- 0.60 \\
10.0--17.7 & 0.37 +/-- 0.04 & 0.39 +/-- 0.05 & 0.37 +/-- 0.06 & 1.45 +/-- 0.55 & 1.19 +/-- 0.27 & 1.74 +/-- 1.13 \\
17.7--31.6 & 0.21 +/-- 0.04 & 0.44 +/- 0.26 & 0.24 +/-- 0.05 & 0.79 +/-- 0.55 & 1.37 +/-- 0.68 & 1.12 +/-- 0.82 \\
31.6--100.0 & 0.37 +/-- 0.43 & -- & 0.19 +/-- 0.02 & 1.94 +/-- 1.57 & -- & 0.62 +/-- 0.24 \\
\hline
\end{tabular} 
\tablecomments{$R_{X}^1$ is the X\% containment radius determined by the stacking analysis. $R_{X}^2$ is the containment determined by background subtraction.}
\end{center}
\end{table}

==> Tables/front.tex <==
\begin{table}[8]\footnotesize
\begin{center}
\caption{Front PSF parameters}
\begin{tabular}{|l|rcrrrrrr|}
\hline
\multicolumn{9}{|c|}{1.0--1.7 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 22374 & 4993 & 0.163 & 1.90 & 0.51 & 0.48 & 1.64 & 1.22 \\
Geminga & 11147 & 1360  & 0.168 & 2.00 & 0.49 & 0.49 & 1.47 & 1.19 \\
Crab & 2743 & 2328 & 0.169 & 2.10 & 0.47 & 0.50 & 1.31 & 1.28 \\
All Pulsars & 36271 & 8675 & 0.165 & 1.94 & 0.50 & -- & 1.56 & -- \\
AGN & 3635 & 24103 & 0.163 & 1.96 & 0.49 & -- & 1.49 & -- \\
\hline
\multicolumn{9}{|c|}{1.7--3.2 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 11229 & 2310 & 0.117 & 2.06 & 0.33 & 0.31 & 0.94 & 0.76 \\
Geminga & 6010 & 682 & 0.119 & 2.25 & 0.31 & 0.31 & 0.80 & 0.69 \\
Crab & 1417 & 1075 & 0.117 & 2.26 & 0.30 & 0.30 & 0.78 & 0.65 \\
All Pulsars & 18664 & 4059 & 0.117 & 2.12 & 0.32 & -- & 0.88 & --\\
AGN & 2266 & 10834 & 0.115 & 2.12 & 0.31 & -- & 0.87 & -- \\
\hline
\multicolumn{9}{|c|}{3.2--5.6 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 4431 &950 & 0.085 & 2.29 & 0.22 & 0.21 & 0.55 & 0.50 \\
Geminga & 2276 & 245 & 0.090 & 2.45 & 0.22 & 0.21 & 0.52 & 0.50 \\
Crab & 626 & 426 & 0.094 & 2.84 & 0.21 & 0.20 & 0.45 & 0.43 \\
All Pulsars & 7321 & 1628 & 0.088 & 2.39 & 0.22 & -- & 0.53 & -- \\
AGN & 1338 & 4814 & 0.078 & 2.10 & 0.22 & -- & 0.60 & -- \\
\hline
\multicolumn{9}{|c|}{5.6--10.0 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 1349 & 382 & 0.059 & 1.93 & 0.18 & 0.18 & 0.57 & 0.49 \\
Geminga & 590 & 107 & 0.080 & 2.50 & 0.19 & 0.20 & 0.45 & 0.42 \\
Crab & 273 & 182 & 0.071 & 2.62 & 0.16 &  0.15 & 0.38 & 0.37 \\
All & 2207 & 681 & 0.065 & 2.11 & 0.18 & -- & 0.50 & -- \\
AGN & 822 & 2117 & 0.062 & 2.01 & 0.18 & -- & 0.53 & -- \\
\hline
\multicolumn{9}{|c|}{10.0--17.7 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 272 & 158 & 0.055 & 1.95 & 0.17 & 0.16 & 0.51 & 0.36 \\
Geminga & 77 & 43 & 0.056 & 2.57 & 0.13 & 0.13 & 0.30 & 0.29 \\
Crab & 144 & 50 & 0.050 & 2.04 & 0.14 & 0.12 & 0.41 & 0.30 \\
All Pulsars& 491 & 253 & 0.053 & 2.05 & 0.15 & -- & 0.44 & -- \\
AGN & 509 & 969 & 0.052 & 2.14 & 0.14 & -- & 0.39 & -- \\
\hline
\multicolumn{9}{|c|}{17.7--31.6 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & 45 & 86 & 0.042 & 2.43 & 0.10 & 0.11 & 0.25 & 0.41 \\
Geminga & 13 & 21 & 0.068 & 2.42 & 0.17 & 0.21 & 0.40 & 0.34 \\
Crab & 66 & 29 & 0.031 & 1.91 & 0.10 & 0.12 & 0.31 & 0.19 \\
All Pulsars & 124 & 136 & 0.037 & 2.03 & 0.11 & -- & 0.31 & -- \\
AGN & 323 & 493 & 0.033 & 1.80 & 0.11 & -- & 0.40 & -- \\
\hline
\multicolumn{9}{|c|}{31.6--100.0 GeV} \\
\hline
Source & $N_{psf}$ & $N_{diff}$ + $N_{iso}$ & $\sigma (deg)$ & $\gamma$ & $R_{68}^1 (deg)$ & $R_{68}^2 (deg)$ & $R_{95}^1 (deg)$ & $R_{95}^2 (deg)$ \\
\hline
Vela & -- & -- & -- & -- & -- & -- & -- & -- \\
Geminga & -- & -- & -- & -- & -- & -- & -- & -- \\
Crab & 36 & 33 & 0.034 & 2.10 & 0.09 & -- & 0.26 & -- \\
All Pulsars & 48 & 106 & 0.028 & 1.55 & 0.13 & -- & 0.73 & -- \\
AGN & 277 & 431 & 0.022 & 1.67 & 0.09 & -- & 0.38 & -- \\
\hline
\end{tabular}
\tablecomments{$R_{X}^1$ is the X\% containment radius determined by the stacking analysis. $R_{X}^2$ is the containment determined by background subtraction.}
\end{center}
\end{table}

==> Tables/halo_1es.tex <==
\begin{deluxetable}{lclc}
\tabletypesize{\scriptsize}

\tablecaption{Energy flux limits for the TeV source 1ES 0229+200 with the convolved Disk and Gaussian models from equations \ref{eq:gausshalo} and \ref{eq:diskhalo} \label{TABLE::1es0229}}

\tablewidth{0pt}
\tablehead{
%&\multicolumn{4}{c}{Low redshift $(z<0.5)$}&\multicolumn{4}{c}{High redshift $(z>0.5)$}\\
%\cline{2-5}\cline{6-8}\\
\colhead{Energy Bin [MeV]} & Halo Size [deg] & Model & 95\%  Energy Flux Upper Limit [ergs cm$^{-2}$ s$^{-1}$]
}
\startdata

1000-1778 & 0.1 & Disk & 5.49e-13 \\
 & 0.1 & Gaussian & 5.73e-13 \\
 & 0.5 & Disk & 7.49e-13 \\
 & 0.5 & Gaussian & 1.22e-12 \\
 & 1.0 & Disk & 1.35e-12 \\
 & 1.0 & Gaussian & 3.25e-12 \\
1778-3162 & 0.1 & Disk & 1.44e-12 \\
 & 0.1 & Gaussian & 1.55e-12 \\
 & 0.5 & Disk & 1.62e-12 \\
 & 0.5 & Gaussian & 2.92e-12 \\
 & 1.0 & Disk & 3.64e-12 \\
 & 1.0 & Gaussian & 8.86e-12 \\
3162-5623 & 0.1 & Disk & 1.37e-12 \\
 & 0.1 & Gaussian & 1.44e-12 \\
 & 0.5 & Disk & 2.37e-12 \\
 & 0.5 & Gaussian & 3.24e-12 \\
 & 1.0 & Disk & 3.20e-12 \\
 & 1.0 & Gaussian & 3.19e-12 \\
5623-10000 & 0.1 & Disk & 1.23e-12 \\
 & 0.1 & Gaussian & 1.28e-12 \\
 & 0.5 & Disk & 2.41e-12 \\
 & 0.5 & Gaussian & 2.69e-12 \\
 & 1.0 & Disk & 2.77e-12 \\
 & 1.0 & Gaussian & 2.76e-12 \\
10000-17783 & 0.1 & Disk & 1.80e-12 \\
 & 0.1 & Gaussian & 1.80e-12 \\
 & 0.5 & Disk & 1.80e-12 \\
 & 0.5 & Gaussian & 1.80e-12 \\
 & 1.0 & Disk & 1.80e-12 \\
 & 1.0 & Gaussian & 1.80e-12 \\
17783-31623 & 0.1 & Disk & 4.36e-12 \\
 & 0.1 & Gaussian & 3.82e-12 \\
 & 0.5 & Disk & 3.16e-12 \\
 & 0.5 & Gaussian & 3.12e-12 \\
 & 1.0 & Disk & 3.10e-12 \\
 & 1.0 & Gaussian & 3.09e-12 \\
31623-100000 & 0.1 & Disk & 7.66e-12 \\
 & 0.1 & Gaussian & 7.68e-12 \\
 & 0.5 & Disk & 7.64e-12 \\
 & 0.5 & Gaussian & 7.66e-12 \\
 & 1.0 & Disk & 7.67e-12 \\
 & 1.0 & Gaussian & 7.62e-12 \\

\enddata
\end{deluxetable}

\begin{deluxetable}{lclc}
\tabletypesize{\scriptsize}

\tablecaption{Energy flux limits for the TeV source 1ES 0347-121 \label{TABLE::1es0347} }

\tablewidth{0pt}
\tablehead{
%&\multicolumn{4}{c}{Low redshift $(z<0.5)$}&\multicolumn{4}{c}{High redshift $(z>0.5)$}\\
%\cline{2-5}\cline{6-8}\\
\colhead{Energy Bin [MeV]} & Halo Size [deg] & Model & 95\%  Energy Flux Upper Limit [ergs cm$^{-2}$ s$^{-1}$]
}
\startdata

1000-1778 & 0.1 & Disk & 6.59e-13 \\
 & 0.1 & Gaussian & 6.76e-13 \\
 & 0.5 & Disk & 7.63e-13 \\
 & 0.5 & Gaussian & 9.69e-13 \\
 & 1.0 & Disk & 9.31e-13 \\
 & 1.0 & Gaussian & 2.20e-12 \\
1778-3162 & 0.1 & Disk & 6.93e-13 \\
 & 0.1 & Gaussian & 7.23e-13 \\
 & 0.5 & Disk & 8.94e-13 \\
 & 0.5 & Gaussian & 1.76e-12 \\
 & 1.0 & Disk & 2.43e-12 \\
 & 1.0 & Gaussian & 6.30e-12 \\
3162-5623 & 0.1 & Disk & 1.52e-12 \\
 & 0.1 & Gaussian & 1.62e-12 \\
 & 0.5 & Disk & 2.71e-12 \\
 & 0.5 & Gaussian & 3.94e-12 \\
 & 1.0 & Disk & 3.97e-12 \\
 & 1.0 & Gaussian & 3.95e-12 \\
5623-10000 & 0.1 & Disk & 1.22e-12 \\
 & 0.1 & Gaussian & 1.22e-12 \\
 & 0.5 & Disk & 1.22e-12 \\
 & 0.5 & Gaussian & 1.22e-12 \\
 & 1.0 & Disk & 1.22e-12 \\
 & 1.0 & Gaussian & 1.22e-12 \\
10000-17783 & 0.1 & Disk & 1.95e-12 \\
 & 0.1 & Gaussian & 1.95e-12 \\
 & 0.5 & Disk & 1.95e-12 \\
 & 0.5 & Gaussian & 1.95e-12 \\
 & 1.0 & Disk & 1.95e-12 \\
 & 1.0 & Gaussian & 1.95e-12 \\
17783-31623 & 0.1 & Disk & 3.34e-12 \\
 & 0.1 & Gaussian & 3.34e-12 \\
 & 0.5 & Disk & 3.34e-12 \\
 & 0.5 & Gaussian & 3.34e-12 \\
 & 1.0 & Disk & 3.34e-12 \\
 & 1.0 & Gaussian & 3.34e-12 \\
31623-100000 & 0.1 & Disk & 8.29e-12 \\
 & 0.1 & Gaussian & 8.31e-12 \\
 & 0.5 & Disk & 8.27e-12 \\
 & 0.5 & Gaussian & 8.29e-12 \\
 & 1.0 & Disk & 8.29e-12 \\
 & 1.0 & Gaussian & 8.24e-12 \\

\enddata
\end{deluxetable}

\begin{deluxetable}{lclc}
\tabletypesize{\scriptsize}

\tablecaption{Energy flux limits for the TeV source 1ES1101-232 \label{TABLE::1es1101}}

\tablewidth{0pt}
\tablehead{
%&\multicolumn{4}{c}{Low redshift $(z<0.5)$}&\multicolumn{4}{c}{High redshift $(z>0.5)$}\\
%\cline{2-5}\cline{6-8}\\
\colhead{Energy Bin [MeV]} & Halo Size [deg] & Model & 95\% Energy Flux Upper Limit [ergs cm$^{-2}$ s$^{-1}$]
}
\startdata

1000-1778 & 0.1 & Disk & -0.00e+00 \\
 & 0.1 & Gaussian & 1.03e-12 \\
 & 0.5 & Disk & 1.11e-12 \\
 & 0.5 & Gaussian & 1.59e-12 \\
 & 1.0 & Disk & 1.57e-12 \\
 & 1.0 & Gaussian & 3.83e-12 \\
1778-3162 & 0.1 & Disk & 7.76e-13 \\
 & 0.1 & Gaussian & 8.26e-13 \\
 & 0.5 & Disk & 1.19e-12 \\
 & 0.5 & Gaussian & 2.43e-12 \\
 & 1.0 & Disk & 3.45e-12 \\
 & 1.0 & Gaussian & 8.48e-12 \\
3162-5623 & 0.1 & Disk & 2.15e-12 \\
 & 0.1 & Gaussian & 2.23e-12 \\
 & 0.5 & Disk & 3.17e-12 \\
 & 0.5 & Gaussian & 3.84e-12 \\
 & 1.0 & Disk & 3.65e-12 \\
 & 1.0 & Gaussian & 3.62e-12 \\
5623-10000 & 0.1 & Disk & 1.93e-12 \\
 & 0.1 & Gaussian & 2.01e-12 \\
 & 0.5 & Disk & 2.82e-12 \\
 & 0.5 & Gaussian & 2.83e-12 \\
 & 1.0 & Disk & 2.66e-12 \\
 & 1.0 & Gaussian & 2.71e-12 \\
10000-17783 & 0.1 & Disk & 1.88e-12 \\
 & 0.1 & Gaussian & 1.88e-12 \\
 & 0.5 & Disk & 1.88e-12 \\
 & 0.5 & Gaussian & 1.88e-12 \\
 & 1.0 & Disk & 1.88e-12 \\
 & 1.0 & Gaussian & 1.88e-12 \\
17783-31623 & 0.1 & Disk & 3.23e-12 \\
 & 0.1 & Gaussian & 3.23e-12 \\
 & 0.5 & Disk & 3.23e-12 \\
 & 0.5 & Gaussian & 3.23e-12 \\
 & 1.0 & Disk & 3.23e-12 \\
 & 1.0 & Gaussian & 3.23e-12 \\
31623-100000 & 0.1 & Disk & 8.02e-12 \\
 & 0.1 & Gaussian & 8.03e-12 \\
 & 0.5 & Disk & 8.06e-12 \\
 & 0.5 & Gaussian & 1.14e-11 \\
 & 1.0 & Disk & 1.10e-11 \\
 & 1.0 & Gaussian & 1.19e-11 \\


\enddata
\end{deluxetable}

==> Tables/halo_TS.tex <==
\begin{deluxetable}{llllllll}
\tabletypesize{\scriptsize}

\tablecaption{Summary of the significance of the convolved Disk Halo models for the low and high redshift blazar samples, $z_{cut}=0.5$. The statistics for the halo size with the largest TS=$2\Delta\textrm{log}L$ are displayed on each row. The halo size is also compared with the P6\_v11 68 and 95\% containment radii. The most significant halo components occur when the halo size is either much smaller than the PSF or near the size of the region of interest. \label{TABLE::DISK}}

\tablewidth{0pt}
\tablehead{
%&\multicolumn{4}{c}{Low redshift $(z<0.5)$}&\multicolumn{4}{c}{High redshift $(z>0.5)$}\\
%\cline{2-5}\cline{6-8}\\
\colhead{Energy Bin [MeV]} & Halo Size [deg] & $R_{68} [deg]$ & $R_{95} [deg]$ & $N^{halo}$ & 68\% U.L. & 95\% U.L. & TS
}
\startdata

      1000--1778 [low]  &  0.080   &   0.476  &                 1.298  &       2.5
                  &     2.5  &     2.5  &              0.002  \\
      1000--1778 [high]   &  0.965   &     &           &    0.0
                  &     42.0  &     95.5  &              0.000  \\
      1778--3162 [low] &  0.160  &   0.300  &                 0.818   &                 
                 61.6 &    347.0    &    686.1  &      0.032   \\
      1778--3162 [high] &  0.052  &     &                    &         851.8        
                 &    855.4    &    899.3  &      4.806   \\
      3162--5623 [low] &  0.724  &   0.203  &                 0.556   &         45.3        
                  &   155.4   &    309.3  &      0.117  \\
      3162--5623 [high] &  0.052  &     &                    &         15.3       
                 &    93.3    &    165.8  &      0.042   \\
     5623--10000 [low] &  0.025  &   0.152  &                 0.414   &         651.7        
                  &   654.2   &    692.4  &      1.687  \\
     5623--10000 [high] &  0.125  &     &                    &         5.7       
                 &    62.7    &    121.5  &      0.008   \\
    10000 -17783 [low] &  0.016  &   0.127  &                0.346   &         218.9        
                  &   154.3   &    280.5  &      1.598  \\
    10000--17783 [high] &  0.060  &     &                    &         97.4       
                 &    101.6    &    115.2  &      8.320   \\
    17783 -31623 [low] &  0.429  &   0.116  &                0.316   &         18.4
                  &  21.0   &    41.3  &      0.308  \\
    17783--31623 [high] & 0.429  &     &                    &        3.2    
                 &    5.4    &    11.1  &      0.120   \\
\enddata
\end{deluxetable}

\begin{deluxetable}{llllllll}
\tabletypesize{\scriptsize}

\tablecaption{Summary of the significance of the convolved Gaussian Halo models for the low and high redshift blazar samples, $z_{cut}=0.5$. The statistics for the halo size with the largest TS=$2\Delta\textrm{log}L$ are displayed on each row. The halo size is also compared with the P6\_v11 68 and 95\% containment radii. \label{TABLE::HALO}}

\tablewidth{0pt}
\tablehead{
%&\multicolumn{4}{c}{Low redshift $(z<0.5)$}&\multicolumn{4}{c}{High redshift $(z>0.5)$}\\
%\cline{2-5}\cline{6-8}\\
\colhead{Energy Bin [MeV]} & Halo Size [deg] & $R_{68} [deg]$ & $R_{95} [deg]$ & $N^{halo}$ & 68\% U.L. & 95\% U.L. & TS
}
\startdata

      1000--1778 [low]  &  0.611   &   0.476  &                 1.298  &      0.0
                  &    45.5  &     113.7  &              0.000  \\
      1000--1778 [high]   &  0.434   &     &           &    0.0
                  &     50.3  &     115.3  &              0.000  \\
      1778--3162 [low] &  0.160  &   0.300  &                 0.818   &      6.9           
                  &    6.9   &    6.9  &      0.008   \\
      1778--3162 [high] &  0.052  &     &                    &        618.5      
                 &   418.9    &    760.1  &      2.595   \\
      3162--5623 [low] &  0.724  &   0.203  &                 0.556   &         121.8    
                  &    800.5    &    951.9  &      0.107  \\
      3162--5623 [high] &  0.586  &     &                    &         18.1       
                 &    82.3  &    155.1  &      0.020   \\
     5623--10000 [low] &  0.025  &   0.152  &                 0.414   &        478.8       
                  &   322.3   &    584.9  &      0.782  \\
     5623--10000 [high] &  0.025  &     &                    &         0.1       
                 &    0.1    &    0.1  &      0.000   \\
    10000 -17783 [low] &  0.017  &   0.127  &                0.346   &         199.7        
                  &   151.7   &    280.9  &      1.382  \\
    10000--17783 [high] &  0.017  &     &                    &         96.6      
                 &   100.9   &    114.4  &      8.137   \\
    17783 -31623 [low] &  0.429  &   0.116  &                0.316   &         19.0
                  &  19.5   &    38.9  &      0.308  \\
    17783--31623 [high] & 0.429  &     &                    &        2.9    
                 &    4.9    &    10.0  &      0.176   \\
\enddata
\end{deluxetable}



==> Tables/phase.tex <==
\begin{table}[8]\footnotesize
\begin{center}
  \caption{On- and off-pulse phase selection and phase interval ratio
    ($\alpha$) for Vela and Geminga pulsars. \label{TABLE::PULSAR_PHASE}}
\begin{tabular}{|llll|}
\hline
Source & On-pulse & Off-pulse & $\alpha$
\hline
Vela & 0.1--0.15, 0.5--0.6 & 0.7--0.1 & 2
Geminga & 0.1--0.17, 0.6--0.68 & 0.25--0.55 & 2
\hline
\end{tabular}
\end{center}
\end{table}

==> Tables/psfagn.tex <==
\begin{deluxetable}{lrrrrrrr}
\tabletypesize{\scriptsize}
  \tablecaption{List of AGN used for calibration of the \irf{P6\_V11} PSF with properties determined by \citet{REF:2010.1FGL}.}
\tablewidth{0pt}
\tablehead{\colhead{Source} & \colhead{R. A.} & \colhead{Dec} &  \colhead{$l$} &  \colhead{$b$} & \colhead {Photon Index} & \colhead{Flux & \colhead{$\sqrt{TS}$\tablenotemark{b}}}
\startdata
1FGL J2253.9+1608 & 343.4948 & 16.1495 & 86.1169 & $-$38.1851 & 2.47 & 46.2 & 85 \\
1FGL J1104.4+3812 & 166.1247 & 38.2108 & 179.8211 & 65.0392 & 1.81 & 26.1 & 76 \\
1FGL J0538.8$-$4404 & 84.7183 & $-$44.0807 & 250.0783 & $-$31.0827 & 2.27 & 21.3 & 53 \\
1FGL J1504.4+1029 & 226.1023 & 10.4927 & 11.3786 & 54.5810 & 2.22 & 67.0 & 113 \\
1FGL J0428.6$-$3756 & 67.1567 & $-$37.9412 & 240.7109 & $-$43.6273 & 2.13 & 25.7 & 63 \\
1FGL J2158.8$-$3013 & 329.7117 & $-$30.2176 & 17.7431 & $-$52.2407 & 1.91 & 27.1 & 70 \\
1FGL J1224.7+2121 & 186.1988 & 21.3634 & 255.0270 & 81.6300 & 2.55 & 2.5 & 13 \\
1FGL J1555.7+1111 & 238.9383 & 11.1921 & 21.9174 & 43.9570 & 1.66 & 13.7 & 51 \\
1FGL J0457.0$-$2325 & 74.2595 & $-$23.4228 & 223.7193 & $-$34.9024 & 2.21 & 32.5 & 73 \\
1FGL J1256.2$-$0547 & 194.0533 & $-$5.7911 & 305.1174 & 57.0603 & 2.32 & 32.4 & 72 \\
1FGL J0319.7+4130 & 49.9413 & 41.5085 & 150.5721 & $-$13.2676 & 2.13 & 17.3 & 45 \\
1FGL J0238.6+1637 & 39.6689 & 16.6214 & 156.7751 & $-$39.1018 & 2.14 & 32.7 & 72 \\
1FGL J0449.5$-$4350 & 72.3783 & $-$43.8384 & 248.8094 & $-$39.9003 & 1.95 & 11.1 & 40 \\
1FGL J1426.9+2347 & 216.7495 & 23.7987 & 29.4830 & 68.2090 & 1.83 & 10.2 & 40 \\
1FGL J0808.2$-$0750 & 122.0543 & $-$7.8399 & 229.0254 & 13.1606 & 2.14 & 10.0 & 32 \\
1FGL J0730.3$-$1141 & 112.5814 & $-$11.6996 & 227.7804 & 3.1360 & 2.33 & 20.7 & 44 \\
1FGL J1802.5$-$3939 & 270.6359 & $-$39.6617 & 352.4424 & $-$8.3938 & 2.25 & 10.4 & 24 \\
1FGL J0957.7+5523 & 149.4315 & 55.3922 & 158.5782 & 47.9361 & 2.05 & 10.5 & 40 \\
1FGL J1522.1+3143 & 230.5450 & 31.7321 & 50.1548 & 57.0194 & 2.42 & 15.9 & 48 \\
1FGL J1015.1+4927 & 153.7885 & 49.4526 & 165.4963 & 52.7181 & 1.93 & 8.7 & 36 \\
1FGL J0303.5$-$2406 & 45.8890 & $-$24.1124 & 214.6189 & $-$60.1500 & 1.98 & 4.6 & 23 \\
1FGL J1312.4+4827 & 198.1098 & 48.4533 & 113.4894 & 68.2881 & 2.34 & 1.5 & 9 \\
1FGL J1457.5$-$3540 & 224.3761 & $-$35.6753 & 329.8938 & 20.5114 & 2.27 & 16.9 & 40 \\
1FGL J0136.5+3905 & 24.1305 & 39.0856 & 132.4155 & $-$22.9545 & 1.73 & 4.5 & 24 \\
1FGL J0818.2+4222 & 124.5522 & 42.3816 & 178.2236 & 33.3920 & 2.15 & 8.7 & 32 \\
1FGL J2202.8+4216 & 330.7155 & 42.2792 & 92.6119 & $-$10.4559 & 2.38 & 7.3 & 21 \\
1FGL J1542.9+6129 & 235.7442 & 61.4860 & 95.3748 & 45.3959 & 2.14 & 5.2 & 25 \\
1FGL J0719.3+3306 & 109.8461 & 33.1113 & 185.0585 & 19.8628 & 2.15 & 6.9 & 26 \\
1FGL J2000.0+6508 & 300.0215 & 65.1334 & 97.9940 & 17.6546 & 2.10 & 6.0 & 26 \\
1FGL J2025.6$-$0735 & 306.4174 & $-$7.5986 & 36.8963 & $-$24.3861 & 2.35 & 12.5 & 36 \\
1FGL J1923.5$-$2104 & 290.8849 & $-$21.0771 & 17.1780 & $-$16.2559 & 2.17 & 11.9 & 33 \\
1FGL J0920.9+4441 & 140.2412 & 44.6888 & 175.7142 & 44.8148 & 2.28 & 14.0 & 44 \\
1FGL J1221.5+2814 & 185.3897 & 28.2467 & 201.6110 & 83.2931 & 2.06 & 6.9 & 29 \\
1FGL J2139.3$-$4235 & 324.8494 & $-$42.5880 & 358.3194 & $-$48.3256 & 2.08 & 8.3 & 29 \\
1FGL J1058.6+5628 & 164.6698 & 56.4801 & 149.5719 & 54.4229 & 1.97 & 5.7 & 30 \\
1FGL J1517.8$-$2423 & 229.4538 & $-$24.3846 & 340.6971 & 27.5517 & 2.10 & 5.6 & 21 \\
1FGL J2009.5$-$4849 & 302.3761 & $-$48.8295 & 350.3773 & $-$32.6141 & 1.90 & 5.0 & 21 \\
1FGL J1246.7$-$2545 & 191.6827 & $-$25.7620 & 301.6038 & 37.0976 & 2.31 & 8.3 & 26 \\
1FGL J0738.2+1741 & 114.5638 & 17.6982 & 201.8669 & 18.0968 & 2.02 & 4.4 & 20 \\
1FGL J0217.9+0144 & 34.4800 & 1.7466 & 162.1781 & $-$54.3988 & 2.18 & 6.0 & 25 \\
1FGL J2056.3$-$4714 & 314.0851 & $-$47.2384 & 352.6010 & $-$40.3934 & 2.54 & 4.8 & 18 \\
1FGL J2203.5+1726 & 330.8824 & 17.4387 & 75.6957 & $-$29.6413 & 2.39 & 4.3 & 18 \\
1FGL J0507.9+6738 & 76.9931 & 67.6367 & 143.7857 & 15.9000 & 1.75 & 2.3 & 17 \\
1FGL J0630.9$-$2406 & 97.7472 & $-$24.1067 & 232.6821 & $-$14.9885 & 1.87 & 3.1 & 17 \\
1FGL J0120.5$-$2700 & 20.1315 & $-$27.0158 & 213.5949 & $-$83.5244 & 1.99 & 3.7 & 20 \\
1FGL J1248.2+5820 & 192.0575 & 58.3365 & 123.7443 & 58.7867 & 2.18 & 4.5 & 23 \\
1FGL J0033.5$-$1921 & 8.3913 & $-$19.3650 & 94.1485 & $-$81.2205 & 1.89 & 2.8 & 16 \\
1FGL J0423.2$-$0118 & 65.8001 & $-$1.3088 & 195.2465 & $-$33.1352 & 2.42 & 5.8 & 22 \\
1FGL J1444.0$-$3906 & 221.0052 & $-$39.1160 & 325.6673 & 18.7345 & 1.83 & 3.5 & 16 \\
1FGL J1253.0+5301 & 193.2646 & 53.0245 & 122.3740 & 64.1020 & 2.14 & 3.2 & 16 \\
1FGL J0137.0+4751 & 24.2506 & 47.8521 & 130.7944 & $-$14.3228 & 2.34 & 9.7 & 30 \\
1FGL J1725.0+1151 & 261.2670 & 11.8573 & 34.1063 & 24.4701 & 1.89 & 3.4 & 16 \\
1FGL J0509.3+0540 & 77.3446 & 5.6746 & 195.4151 & $-$19.6570 & 2.16 & 3.9 & 18 \\
1FGL J1903.0+5539 & 285.7726 & 55.6505 & 85.9343 & 20.5450 & 1.86 & 3.6 & 17 \\
1FGL J1344.2$-$1723 & 206.0712 & $-$17.3925 & 320.4820 & 43.6710 & 2.11 & 6.0 & 21 \\
1FGL J0221.0+3555 & 35.2708 & 35.9308 & 142.6031 & $-$23.4932 & 2.33 & 6.4 & 26 \\
1FGL J1058.4+0134 & 164.6200 & 1.5815 & 251.4899 & 52.7827 & 2.29 & 7.1 & 27 \\
1FGL J0700.4$-$6611 & 105.1008 & $-$66.1891 & 276.7764 & $-$23.7733 & 2.15 & 4.7 & 19 \\
1FGL J1159.4+2914 & 179.8531 & 29.2439 & 199.4383 & 78.3492 & 2.37 & 5.5 & 23 \\
1FGL J0334.4$-$3727 & 53.6028 & $-$37.4662 & 240.2139 & $-$54.3471 & 2.10 & 2.8 & 13 \\
1FGL J0825.8$-$2230 & 126.4678 & $-$22.5104 & 243.9726 & 8.8993 & 2.14 & 5.3 & 22 \\
1FGL J1917.7$-$1922 & 289.4371 & $-$19.3668 & 18.2332 & $-$14.3233 & 1.88 & 3.3 & 15 \\
1FGL J0442.7$-$0019 & 70.6894 & $-$0.3191 & 197.2391 & $-$28.4498 & 2.44 & 6.3 & 24 \\
1FGL J2329.2$-$4954 & 352.3180 & $-$49.9028 & 332.0478 & $-$62.3242 & 2.42 & 4.2 & 17 \\
1FGL J0433.5+2905 & 68.3887 & 29.0893 & 170.5161 & $-$12.6205 & 2.13 & 4.5 & 16 \\

\enddata
\tablenotetext{a}{Photon flux for 1 GeV-100 GeV obtained by summing the photon flux values from the likelihood analysis in the three bands from 1 GeV to 100 GeV. ($10^{-9} ~ \textrm{photons} ~ \textrm{cm}^{-2}\textrm{s}^{-1}$)}
\tablenotetext{b}{Sum of the $TS$ from the likelihood analysis in the three bands from 1 GeV to 100 GeV.}
\label{TABLE::PSFAGN}
\end{deluxetable}
